Kernel KMeans clustering splits for end-to-end unsupervised decision trees

Trees are convenient models for obtaining explainable predictions on relatively small datasets. Although there are many proposals for the end-to-end construction of such trees in supervised learning, learning a tree end-to-end for clustering without labels remains an open challenge. As most works focus on interpreting with trees the result of another clustering algorithm, we present here a novel end-to-end trained unsupervised binary tree for clustering: Kauri. This method performs a greedy maximisation of the kernel KMeans objective without requiring the definition of centroids. We compare this model on multiple datasets with recent unsupervised trees and show that Kauri performs identically when using a linear kernel. For other kernels, Kauri often outperforms the concatenation of kernel KMeans and a CART decision tree.

==> figs_tex/fig_digits_mice.tex <==
\begin{figure}
    \centering
    %\subfloat[][Mice clustering]{\includegraphics[width=0.2\linewidth]{figs/mice_ari.pdf}\label{sfig:mice_ari}}\hfil
    \subfloat[][Mice]{\includegraphics[width=0.3\textwidth]{figs/mice_waes.pdf}\label{sfig:mice_waes}}\hfil
    %\subfloat[][Digits clustering]{\includegraphics[width=0.2\linewidth]{figs/digits_ari.pdf}\label{sfig:digits_ari}}\hfil
    \subfloat[][Digits]{\includegraphics[width=0.3\textwidth]{figs/digits_waes.pdf}\label{sfig:digits_waes}}\hfil
    \caption{Explanation scoring with WAES (lower is better) as the maximal number of leaves increases on the mice protein and digits datasets for Kauri (green), KMeans+Tree (blue) and ExKMC (red).}
    \label{fig:mice_digits}
\end{figure}

==> figs_tex/fig_gap_stats.tex <==
\begin{figure}
    \centering
    \subfloat[][Iris (?/?)]{\includegraphics[width=0.2\linewidth]{figs/iris_Gap.pdf}\label{sfig:iris_gap}}\hfil
    \subfloat[][Haberman's survival (5/4)]{\includegraphics[width=0.2\linewidth]{figs/haberman_survival_Gap.pdf}\label{sfig:haberman_gap}}\hfil
    \subfloat[][Breast cancer Wisconsin (?/?)]{\includegraphics[width=0.2\linewidth]{figs/breast_cancer_Gap.pdf}\label{sfig:breast_cancer_gap}}\hfil
    \subfloat[][Mice protein expression (?/?)]{\includegraphics[width=0.2\linewidth]{figs/mice_protein_Gap.pdf}\label{sfig:mice_gap}}
    \caption{Gap statistic curves of Kauri various numbers of clusters compared with the KMeans+Tree algorithm. The selected number of clusters are written in parentheses as (Kauri / KMeans+Tree). We wrote ? when we were unable to determine a relevant gap within the limit of one standard deviation.}
    \label{fig:gap_scores}
\end{figure}

==> figs_tex/fig_qualitative_comparison.tex <==
\begin{figure}
\subfloat[KAURI]{
\includegraphics[width=0.3\linewidth]{figs/qualitative_plot_kauri.pdf}
\label{sfig:kauri_boudary_target}
}
\subfloat[Kernel KMeans]{
\includegraphics[width=0.3\linewidth]{figs/qualitative_plot_kmeans.pdf}
\label{sfig:kmeans_boudary_target}
}
\subfloat[Kernel KMeans + Decision Tree]{
\includegraphics[width=0.3\linewidth]{figs/qualitative_plot_ktree.pdf}
\label{sfig:ktree_boudary_target}
}
\caption{Decision boundaries for the RBF kernel on two concentric circles. The respective kernel KMeans scores are (a) $1.501\times10^6$ (b) $1.508\times 10^6$ (c) $1.685\times 10^6$. Both trees are constrained to two leaves.}
\label{fig:tree_boundary_target}
\end{figure}

==> figs_tex/fig_silhouette_scores.tex <==
\begin{figure}
    \centering
    \subfloat[][Iris (2/2/11)]{\includegraphics[width=0.2\linewidth]{figs/iris_Silhouette.pdf}\label{sfig:iris_silhouette}}\hfil
    \subfloat[][Haberman's survival (3/3/2)]{\includegraphics[width=0.2\linewidth]{figs/haberman_survival_Silhouette.pdf}\label{sfig:haberman_silhouette}}\hfil
    \subfloat[][Breast cancer Wisconsin (2/2/4)]{\includegraphics[width=0.2\linewidth]{figs/breast_cancer_Silhouette.pdf}\label{sfig:breast_cancer_silhouette}}\hfil
    \subfloat[][Mice protein expression (13/13/13)]{\includegraphics[width=0.2\linewidth]{figs/mice_protein_Silhouette.pdf}\label{sfig:mice_silhouette}}
    \caption{Silhouette scores of Kauri and Douglas for various numbers of clusters compared with the KMeans+Tree algorithm. Selected number of clusters are written in parentheses as (Kauri / KMeans+Tree / Douglas).}
    \label{fig:silhouette_scores}
\end{figure}

==> figs_tex/tab_benchmark_small_kmeans.tex <==
\begin{table*}[!th]
    \centering
    \caption{Relative KMeans score \std{std} (lower is better) after 30 runs on subsamples of 80\% of the input datasets divided by the KMeans reference score (=1.0). All models are limited to finding as many leaves as clusters.}
    \label{tab:benchmark_small_kmeans}
    \begin{tabular}{ccccccc}
        \toprule
        Dataset & Kauri & KMeans+DT & ICOT & IMM & ExShallow & RDM \\
        \midrule
        Atom & 1.03\std{0.02} & 1.04\std{0.02} & 1.05\std{0.03} & \textbf{1.02\std{0.02}} & 1.04\std{0.02} & 1.03\std{0.02} \\
        %Avila & \textbf{1.45\std{0.58}} & 3.33\std{1.16} & X & 1.49\std{0.66} & 1.52\std{0.71} & 1.99\std{0.68} \\
        Cancer & 1.14\std{0.03} & 1.14\std{0.03} & \textbf{1.09\std{0.04}} & 1.14\std{0.03} & 1.14\std{0.03} & 1.37\std{0.04} \\
        %Car & \textbf{1.00\std{0.00}} & \textbf{1.00\std{0.00}} & X & \textbf{1.00\std{0.00}} & \textbf{1.00\std{0.00}} & 1.02\std{0.03} \\
        Chainlink & \textbf{1.02\std{0.01}} & \textbf{1.02\std{0.01}} & 1.04\std{0.02} & \textbf{1.02\std{0.01}} & \textbf{1.02\std{0.01}} & 1.03\std{0.01} \\
        %Congress & 1.09\std{0.01} & 1.09\std{0.02} & \textbf{1.08\std{0.01}} & 1.09\std{0.01} & 1.09\std{0.02} & 1.19\std{0.02} \\
        Digits & 1.21\std{0.01} & 1.24\std{0.02} & X & 1.25\std{0.02} & \textbf{1.20\std{0.01}} & 1.38\std{0.04} \\
        %Engytime & 1.14\std{0.04} & 1.15\std{0.05} & X & \textbf{1.13\std{0.04}} & 1.14\std{0.06} & 1.15\std{0.05} \\
        %Haberman & 1.10\std{0.07} & \textbf{1.08\std{0.04}} & 1.09\std{0.04} & 1.10\std{0.07} & \textbf{1.08\std{0.04}} & 1.10\std{0.06} \\
        Hepta & 1.09\std{0.09} & 1.08\std{0.03} & 3.12\std{1.94} & \textbf{1.07\std{0.04}} & 1.08\std{0.03} & 1.36\std{0.09} \\
        Iris & 1.18\std{0.06} & 1.19\std{0.05} & 1.92\std{0.10} & 1.17\std{0.05} & \textbf{1.16\std{0.04}} & 1.46\std{0.10} \\
        Lsun & 1.09\std{0.04} & 1.09\std{0.04} & 1.14\std{0.12} & \textbf{1.07\std{0.03}} & \textbf{1.07\std{0.04}} & 1.66\std{0.09} \\
        Mice & \textbf{1.08\std{0.02}} & 1.11\std{0.04} & X & 1.14\std{0.05} & \textbf{1.08\std{0.02}} & 1.41\std{0.06} \\
        Target & 1.35\std{0.05} & 1.58\std{0.13} & X & \textbf{1.19\std{0.08}} & \textbf{1.19\std{0.03}} & 1.83\std{0.10} \\
        %Tetra & 1.12\std{0.15} & \textbf{1.04\std{0.02}} & \textbf{1.04\std{0.01}} & \textbf{1.04\std{0.02}} & 1.05\std{0.02} & 1.53\std{0.06} \\
        %Twodiamonds & 1.05\std{0.02} & \textbf{1.04\std{0.02}} & \textbf{1.04\std{0.02}} & 1.05\std{0.02} & \textbf{1.04\std{0.02}} & \textbf{1.04\std{0.02}} \\
        %Vowel & \textbf{1.07\std{0.01}} & 1.08\std{0.01} & X & 1.09\std{0.02} & \textbf{1.07\std{0.01}} & 1.11\std{0.01} \\
        Wine & 1.15\std{0.05} & 1.15\std{0.08} & 1.37\std{0.17} & \textbf{1.11\std{0.04}} & \textbf{1.11\std{0.04}} & 1.54\std{0.10} \\
        %Wingnut & \textbf{1.09\std{0.02}} & \textbf{1.09\std{0.01}} & 1.14\std{0.06} & \textbf{1.09\std{0.02}} & \textbf{1.09\std{0.02}} & \textbf{1.09\std{0.01}} \\
        \bottomrule
    \end{tabular}
\end{table*}
